Neighborhood Structure Configuration Models

We develop a new method to efficiently sample synthetic networks that preserve the d-hop neighborhood structure of a given network for any given d. The proposed algorithm trades off the diversity in network samples against the depth of the neighborhood structure that is preserved. Our key innovation is to employ a colored Configuration Model with colors derived from iterations of the so-called Color Refinement algorithm. We prove that with increasing iterations the preserved structural information increases: the generated synthetic networks and the original network become more and more similar, and are eventually indistinguishable in terms of centrality measures such as PageRank, HITS, Katz centrality and eigenvector centrality. Our work enables to efficiently generate samples with a precisely controlled similarity to the original network, especially for large networks.

==> contributions.tex <==
Centrality preserving network model
- WL-Lehman based configuration models: Preserving centrality measures across scales?


- Color refinement based configuration models: [Tunable] Network generation (approximately) preserving centrality measures


Local colored configuration models

- microcanonical 

1) Methodische contribution: WL + Configuration models
2) Demonstration of utility: Anwendbarkeit auf Zentralitätsmaße

Narrativ durch die Einleitung?
- Motivation über Centralitätsmaße, Nullmodelle die gewisse Dinger erhalten und alles andere Zufällig lässt, Motifs sind schwer (Exponential random graphs), 
- Motivation über das Zusammenführen

Wir machen neighborhood information preserving color refinement, algorithmen aus der Graph isomophie -> erlaubt uns Netzwerke zu generieren die Zentralitätsmaße approximately erhalten


Main contribution: Introduce framework for graph generation
Calculate WL colors -> use for Colored cofiguration model -> Centralitätsmaße 
Man kann jetzt die ein ähnliches Centralitäts Profil erzeugen


Sub Contribution:
- upper bound on pagerank convergence error
- meta theorem for eigenvector-based centralities (not entirely new)
    - "Once WL has converged a lot of centralities are the same"
- in out WL (needed for HITS)
- framework can be tuned:
  - pagerank-PANICC
  - HITS-PANICC
- diversity?


color refinement configuration model

Wir näher uns mehr und mehr den Farben des WL oder anders gesagt, wir erhalten immer mehr die Nachbarschaftsstrukturen der Knoten


Figure eins: Die extremen Punkte anmarkern (WL preserving auf der einen, Configuration model auf der anderen)


Die Verteilungen über der Zentralitätsmaße konvergieren lassen
Für ein einzelnes Netzwerk die konvergenz einzelner Knoten

The unique idea of our approach is
We demonstrate the utitly of the model by


